You Frame It: How Conceptual Representations Shape LLM Detection and Reasoning about Antisemitism

LLMs enable the integration of external conceptual resources at inference time, creating new opportunities for detecting ideologically and historically complex phenomena such as antisemitism. We investigate how different forms of conceptual grounding affect antisemitism detection and explanation behavior across four state-of-the-art LLMs. Using two expert-annotated datasets, we compare definitional, fine-grained taxonomic, example-augmented, and large-context representations of antisemitism. We find that fine-grained taxonomic representations substantially improve recall, while simultaneously reducing precision. Surprisingly, supplying substantially larger conceptual resources yields no additional quantitative benefit. Post-Holocaust antisemitism poses the most persistent challenge across models and configurations. Analysis of explanations further reveals systematic limitations including overproduction of conceptual references, reliance on lexical cues, overconfidence, and difficulties with subtle or justificatory forms of antisemitism. Our findings highlight both the potential and the remaining limitations of conceptually grounded LLMs for antisemitism detection and reasoning.

==> tables/content_groups_small.tex <==
\begin{table}[t]
\centering
\caption{
Mapping of  Lexicon chapters and IHRA sections to joint content groups.
}
\label{tab:contnet_groups_small}
\small
\setlength{\tabcolsep}{6pt}

\begin{tabular}{lll}
\toprule
\textbf{Content group} 
& \textbf{Lexicon chapters}
& \textbf{IHRA sections} \\
\midrule

Aggressive+Hate
& 37--42
& 0, 1 \\

Classic+Power
& 2--15
& 2, 3, 6 \\

Israel-related 
& 28--36
& 7, 8, 9, 10 \\

Post-Holocaust 
& 16--27
& 4, 5, 11 \\


\bottomrule
\end{tabular}
\end{table}
